Dynamically meeting performance objectives for multiple services on a service mesh

We present a framework that lets a service provider achieve end-to-end management objectives under varying load. Dynamic control actions are performed by a reinforcement learning (RL) agent. Our work includes experimentation and evaluation on a laboratory testbed where we have implemented basic information services on a service mesh supported by the Istio and Kubernetes platforms. We investigate different management objectives that include end-to-end delay bounds on service requests, throughput objectives, and service differentiation. These objectives are mapped onto reward functions that an RL agent learns to optimize, by executing control actions, namely, request routing and request blocking. We compute the control policies not on the testbed, but in a simulator, which speeds up the learning process by orders of magnitude. In our approach, the system model is learned on the testbed; it is then used to instantiate the simulator, which produces near-optimal control policies for various management objectives. The learned policies are then evaluated on the testbed using unseen load patterns.

==> generating_the_system_model.tex <==
\subsection{Generating the system model}
\label{sec:learning_the_system_model}

Learning the effective policy on the real system cause two main challenges, namely infeasible training time and difficulties with investigating the edge cases. To address these challenges, we apply the idea presented in \cite{hammar_stader_journal21}. We develop a framework with two main parts, real system and the simulation of this system (see Figure \ref{fig:simulation_framework}). The procedure in this framework includes the following steps:

\begin{enumerate}
    \item Select a scenario and formulate the RL model
    \item Run the scenario on the testbed and collect monitoring data
    \item Using monitoring data and learn system model (delay model)
    \item Simulate scenario and learn control policy
    \item Evaluate learned policy on \textbf{simulator} on (1) same scenario, (2) modified scenario
    \item Evaluate learned policy on \textbf{testbed} on (1) same scenario, (2) modified scenario
\end{enumerate}

In this procedure, in steps (1-4) we set up the simulation of the real system and use it to learn the effective policy. In step 5, first, we should make sure that the learned policy is effective in the simulation for the load pattern used for learning. To assess the generality of the effective policy, we change the load pattern and evaluate the learned policy. If the learned policy is performing effectively in the simulation environment, we transfer the policy to the real system and evaluate it with two load patterns: 1) the load pattern used for learning and 2) the unseen load pattern. 

\begin{figure}[!htbp]
 \centering
 \includegraphics[scale=0.3]{images/learning_system_model/simulation_framework.png}
 \caption{The developed framework to learn the effective policy on the simulation of the real system.}
 \label{fig:simulation_framework}
\end{figure}

In the above procedure, steps 1-4, we collect data and learn the system model. Since we use this system model to learn the effective policy efficiently, the accuracy and effectiveness of the learned policy are highly related to the accuracy and effectiveness of the system model. We define the system model as $\mathcal{M}:(l_i(t), p_{ij}(t), b_i(t))\longrightarrow d_{ij}(t)$ (see Table \ref{tab:notation} for the notation). 

To produce the delay model ($\mathcal{M}$), we emulate the client populations sending the loads $l_1 \times l_2$ for different combination of actions $p_{11} \times p_{21} \times b_1 \times b_2, \text{where } l_1, l_2 \in \{5,10,15,20\}, p_{11}, p_{21}, b_1, b_2 \in \{0, 0.2, 0.4, ..., 1.0\}$ and measure the response times for each service on each node. Figure \ref{fig:delay_model_3d} shows the measured response times for service $2$ on node $1$. For each pair of loads, we collect $2$ samples of response times for each service for different combinations of loads and actions. After collecting the samples, we use the random forest method to learn the delay model of each service on each node. Figure \ref{fig:predicted_response_times_for_d21} shows the prediction of the response time for service $2$ on node $1$. Table \ref{tab:delay_predictions} shows the accuracy of the learned delay models. We use the average over the training values as the naive estimator. Comparing the error values of the learned model with the naive estimator, we can conclude that the error of the system model is $7\%-10\%$.

\begin{figure}[!htbp]
 \centering
 \includegraphics[scale=0.23]{images/learning_system_model/d21.png}
 \caption{Response time of service $2$ on node $1$ with respect to the offered load of service $1$ and $2$ (to produce this plot, we set the drop rate to $0$, therefore, the carried load is equal to the offered load).}
 \label{fig:delay_model_3d}
\end{figure}

\begin{figure}[!htbp]
 \centering
 \includegraphics[scale=0.29]{images/learning_system_model/d21_predictions.png}
 \caption{Prediction of the response time of service $2$ on node $1$ using the trained delay model. For better visualization, we sample 500 samples randomly from the test set.}
 \label{fig:predicted_response_times_for_d21}
\end{figure}

\begin{table}[!htbp]
\centering
\caption{The accuracy of the response time prediction for the services on the nodes.}
\label{tab:delay_predictions}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Delay} & \multicolumn{2}{c|}{Test} & \multicolumn{1}{c|}{Naive} \\\hhline{~---}
 & $NMAE$ & $R^2$ & $NMAE$\\\hline
$d11$  & $\mathbf{0.103\pm 0.00091}$ & $0.88\pm0.0019$ & $0.419\pm0.0016$ \\
$d12$  & $\mathbf{0.102\pm0.00063}$ & $0.88\pm0.0019$ & $0.414\pm0.0025$ \\
$d21$  & $\mathbf{0.0778\pm 0.00062}$ & $0.91\pm0.0019$ & $0.418\pm0.0022$ \\
$d22$  & $\mathbf{0.0781\pm0.00079}$ & $0.90\pm0.0020$ & $0.417\pm0.0016$ \\\hline

\end{tabular}
\end{table} 

